Investigating Agency of LLMs in Human-AI Collaboration Tasks

Agency, the capacity to proactively shape events, is central to how humans interact and collaborate. While LLMs are being developed to simulate human behavior and serve as human-like agents, little attention has been given to the Agency that these models should possess in order to proactively manage the direction of interaction and collaboration. In this paper, we investigate Agency as a desirable function of LLMs, and how it can be measured and managed. We build on social-cognitive theory to develop a framework of features through which Agency is expressed in dialogue - indicating what you intend to do (Intentionality), motivating your intentions (Motivation), having self-belief in intentions (Self-Efficacy), and being able to self-adjust (Self-Regulation). We collect a new dataset of 83 human-human collaborative interior design conversations containing 908 conversational snippets annotated for Agency features. Using this dataset, we develop methods for measuring Agency of LLMs. Automatic and human evaluations show that models that manifest features associated with high Intentionality, Motivation, Self-Efficacy, and Self-Regulation are more likely to be perceived as strongly agentive.

==> tables/tab_agency_classification.tex <==
\begin{table}
\small
\centering
\def\arraystretch{1.15}
\begin{tabular}
{l|cc}
\toprule
\textbf{Model} & \textbf{Acc.} & \textbf{Macro-F1}  \\
\midrule
DialoGPT & & \\
GPT-3 (Q/A) & & \\
GPT-3 (Fine-tuning) & & \\
GPT-3 (COT) & & \\
\bottomrule
\end{tabular}
% \vspace{-5pt}
\caption{.} 
\label{tab:agency-classification}
\end{table}
